Multimodal Task Vectors Enable Many-Shot Multimodal In-Context Learning

The recent success of interleaved Large Multimodal Models (LMMs) in few-shot learning suggests that in-context learning (ICL) with many examples can be promising for learning new tasks. However, this many-shot multimodal ICL setting has one crucial problem: it is fundamentally limited by the model's context length set at pretraining. The problem is especially prominent in the multimodal domain, which processes both text and images, requiring additional tokens. This motivates the need for a multimodal method to compress many shots into fewer tokens without finetuning. In this work, we enable LMMs to perform multimodal, many-shot in-context learning by leveraging Multimodal Task Vectors (MTV) -- compact implicit representations of in-context examples compressed in the model's attention heads. Specifically, we first demonstrate the existence of such MTV in LMMs and then leverage these extracted MTV to enable many-shot in-context learning for various vision-and-language tasks. Our experiments suggest that MTV can scale in performance with the number of compressed shots and generalize to similar out-of-domain tasks without additional context length for inference. Code: https://github.com/Brandon3964/MultiModal-Task-Vector

==> archive/1_intro_pre_trim.tex <==
\section{Introduction}

%Structure:
% 1. LMMs can do MM-ICL -> limitations to doing it
% 2. Context length
% 3. Describes methods and benefits

% Scaling
\input{figs/fig1_overview}
Large Multimodal Models (LMMs) such as GPT-4V~\cite{OpenAI2023GPT4TR}, LLaVA~\cite{liu2023llava, liu2023llava15}, and the BLIP~\cite{instructblip,li2023blip2} family of models demonstrate state-of-the-art performance on a variety of vision and language tasks thanks to their strong reasoning capabilities over both text and images. Recent works show that LMMs pre-trained on interleaved text-image data may be able to do multimodal in-context learning~\cite{Bai2023QwenVLAF, Laurenccon2024Idefics2}. In particular, few-shot, in-context learning (ICL) in the text-only domain has been scaled with an increasing number of examples in long-context language models---a setting called many-shot learning~\cite{Agarwal2024ManyShotIL}. A natural question thus arises on how to perform many-shot learning in the multimodal domain. 

% First, there is the problem of fitting explicit many-shot examples into a limited context length. 

% This can be in the form of hard limits, increased computing for inference, or less coherent outputs

% A recent focus in research has been on the context length, from extending it to evidence indicating that these models cannot remember the entire context~\cite{Liu2023LostIT}.

% Context length has been a recent focus in research, from trying to extend it to evidence suggesting that these models cannot remember the entire context length~\cite{Liu2023LostIT}.

% Extending the context length requires positional interpolation methods~\cite{Chen2023PosInter, Peng2023YaRNEC}, and even then, there is evidence to suggest that these models cannot remember the entire context length~\cite{Liu2023LostIT}.

% Dealing with this issue has been a recent focu


The first issue with directly applying a many-shot learning regimen to LMMs is the intrinsic limitation of context length. This is especially true in the multimodal domain, as LMMs must encode both text and images, whose embeddings are token-expensive. Moreover, long-context language models, which LMMs leverage for reasoning, struggle to use their entire context length effectively for ICL~\cite{Liu2023LostIT, Li2024LongcontextLS}. Secondly, perhaps due to the misalignment of pretraining tasks with ICL, many instruction-tuned LMMs, even some with interleaved image-text data in their pretraining datasets, underperform on tasks in the ICL setting~\cite{Doveh2024TowardsMM-ICL}. Finally, there is also the challenge of the increasing compute resources and run-time required for processing long contexts for every inference call. These challenges motivate a method for compressing multimodal in-context examples into compact, implicit representations. Therefore, in this paper, we propose {\model} ({\smodel})---compact representations of multimodal in-context tasks---within the attention heads of LMMs to enable many-shot ICL. In particular, we show the existence of {\smodel} in LMMs, and we use them to compress large numbers of multimodal ICL examples, achieving effective many-shot ICL on various vision-and-language tasks.


% Furthermore, we propose leveraging {\smodel} to compress large numbers of multimodal ICL examples to achieve effective many-shot ICL on a variety of vision-and-language tasks.

% However, LMMs struggle to effectively scale few-shot ICL to many-shot learning (i.e., using increasingly higher-order of magnitude number of examples) due to limitations in context length and memory. Thus, we are motivated, in our work, to find a compressed representation that allows us to effectively leverage many examples for in-context learning.

% The practical use of many examples for in-context learning is a key challenge for Large Language Models~\cite{}. However, research in this area is limited primarily by the \textit{context length} of the model. \roei{elaborate...} 
% Additionally, increasing the number of examples also requires increasing amounts of compute resources, lessening the value of learning from examples without finetuning the model. These problems are exacerbated further for Large Multimodal Models that must process both text and image embeddings. Therefore, in this paper, we demonstrate the existence of {\model} ({\smodel})---compact implicit representations of multimodal in-context tasks---within the attention heads of LMMs. Furthermore, we propose leveraging {\smodel} to compress large numbers of multimodal ICL examples to achieve effective many-shot ICL on a variety of vision-and-language tasks.

Recent works in the explainability line of research have demonstrated the existence of task vectors in both the language~\cite{Todd2023FunctionVI, Hendel2023InContextLC} and vision~\cite{Hojel2024FindingVT} domains. These task vectors are implicit representations of an in-context task represented by sets of activations in the model. In our work, we go beyond proving the existence of these task vectors in the multimodal domain and demonstrate their ability to compress examples for many-shot ICL in LMMs without the need for fine-tuning. 

Our method can be described in three steps. First, given a set of many-shot multimodal ICL examples, we calculate the mean activations of the attention heads across multiple inference iterations. Second, to avoid being constrained by the context length, we wish to select a set of attention heads in the model to store the mean activations of the ICL examples. However, since the downstream task may not be in ICL form, we select a set of examples aligned with its form. We then use these examples to find an optimal set of LMM head locations where the many-shot examples will be encoded. We refer to these mean activations and locations as {\smodel}, and in that way, they implicitly encode the many-shot multimodal examples for use in the downstream task. Finally, for downstream inference, we replace the mean activations from Step 1 directly into the attention head locations found in Step 2. 
Since we input examples to the LMM across different iterations in Step 1, {\model} serves as a way to exceed the LMM context limits by implicitly encoding more examples across than allowable by the context limit.
We find that utilizing many examples for extracting {\smodel} in this way surpasses performance on both zero-shot and standard few-shot ICL settings, suggesting the effectiveness of our method. Another key benefit of our method is that it frees up tokens for the model during downstream inference compared to standard few-shot ICL methods.

% since only the query has to be inputted.


% Another key benefit of our method is that it does not require any context length for many-shot ICL, freeing up tokens for the model and leading to more efficient inference compared to standard ICL methods.

To summarize, our main contributions are: (i) We show the existence of {\model}, compact implicit representations of in-context functions in LMMs. (ii) We find that {\smodel} can encode more examples than allowed by an LMM's context length, enabling both token and compute-efficient multimodal many-shot in-context learning.
(iii) {\smodel} surpasses zero-shot and standard few-shot ICL settings without finetuning the LMM on various VL benchmarks. 
(iv) We show that our method can scale to larger numbers of examples and can generalize to similar out-of-domain tasks.

% \roei{When I think of it, I think we should also mention here that this is a new paradigm between ICL and fine-tuning. wdyt? Too much?} 
% CM Response: You are right that this is new for multimodal case, but not generally, so I think we don't need to be explicit about it, otherwise reviewers can make a point out of it for no reason. But in some sense half true!
% \roei{and I think that one important thing to me about this work is the ability not to be limited to context size. This is also not here.}
% Done!


%Contributions:
%


%Recent works presenting LMMs pre-trained on interleaved text-image data ~\cite{Sun2023Emu2, Alayrac2022FlamingoAV, Laurenccon2023IDEFICS, Bai2023QwenVLAF} as well as finetuning existing LMMs to use interleaved images and text~\cite{Doveh2024TowardsMM-ICL} show promise for Multi-Modal In-context Learning (MM-ICL).

% In Large \textit{Language} Models, past work has shown that text-only ICL tasks can be represented implicitly in some subset of the activation heads. Averaged over a set of ICL examples, these \textit{task vectors}~\cite{Todd2023FunctionVI, Hendel2023InContextLC, Hojel2024FindingVT} can be used by LLMs to complete the ICL tasks without additional finetuning or examples. Motivated by these findings, we investigate the existence and application of task vectors extracted from MM-ICL examples.

% Our method---{\model} ({\smodel})---

%Sounding like contributions: don't want to repeat
% show in our work that task vectors also exist for Large Multimodal Models. Further, we show that these task vectors can be used to improve both zero-shot and few-shot performance of LMMs on a variety of VL tasks. Finally, we perform a set of experiments to characterize 

==> archive/2_related_works_pretrim.tex <==
\section{Related Works}


\minisection{Many-Shot In-Context Learning} The promise of learning a task from a set of examples without finetuning makes few-shot, in-context learning an important area of study in LLMs~\cite{Brown2020OGICL,Wei2022EmergentAO}. Similar capabilities have also been demonstrated in the multimodal ICL in Large Multimodal Models~\cite{Sun2023Emu2, Bai2023QwenVLAF, Laurenccon2024Idefics2}. A natural question arises as to the possibility and effectiveness of using a larger number of shots (e.g., hundreds) to further improve performance or learn more complex tasks. Indeed, this emerging area of \textit{many-shot, in-context learning} shows excitingly that performance can scale with larger numbers of examples for a variety of tasks~\cite{Bertsch2024InContextLW, Agarwal2024ManyShotIL, Li2023InContextLW, Li2024LongcontextLS}. 

However, the requirement of long-context models is a significant challenge in and of itself. One method to increase context length in LLMs is to finetune the model with positional interpolation methods~\cite{Chen2023PosInter, Peng2023YaRNEC} applied to the positional encodings of the model. However, research probing the nature of this longer context finds that LLMs---and by extension LMMs---struggle to make use of the entire long context for in-context learning~\cite{Liu2023LostIT, Li2024LongcontextLS}. Moreover, as inference on long contexts of inputs is also computationally and time-expensive, it is unclear whether simply scaling the context of models is an effective and practical method for enabling multimodal many-shot ICL. This has led to work most similar to our own, which looks to compress explicit input tokens~\cite{Ge2023IncontextAF, Tan2024LLoCOLL, ChevalierAutoCOmp, Mu2023LearningTC, Snell2022LearningBD, Jiang2023LLMLinguaCP}. But crucially, these methods either perform finetuning to improve performance or finetune to preserve performance and save inference time and computation. Our work takes a different perspective by focusing on enabling \textit{multimodal} models with many-shot ICL capabilities. Finally, our method improves performance and efficiency on a variety of VL tasks without the use of finetuning.

\minisection{Model Domain Adaptation Methods} 
Commensurate with the development of LLM and LMM model architectures is the progress in methods for generalizing these models to tasks outside of the domain of the pre-training data. The first broad category of these methods involves finetuning some or all of the model. Methods like instruction tuning~\cite{Wei2021FinetunedLM, liu2023llava, avraham2022svit, sanh2022multitask} have shown strong zero-shot generalization to out-of-domain tasks, but forgetting remains an issue. The main proposed solution to this issue involves Parameter Efficient Fine-tuning (PEFT)~\cite{houlsby19adapters}: finetuning either a set of soft prompt input tokens~\cite{Lester2021ThePO, Li2021PrefixTuningOC}, low-rank adaptation of model weights~\cite{Hu2021LoRALA, Dettmers2023QLoRAEF, Zhang2023AdaLoRA}, or learning a separate adapter to the main model~\cite{Zhang2023LLaMAAdapter1, Gao2023LLaMAAdapter2, Hu2023LLMAdaptersAA}.

Nevertheless, prompting methods are a well-explored area for adapting models without finetuning. LLM prompting includes zero-shot methods~\cite{Kojima2022LargeLM, Wang2023PlanandSolvePI, Wan2023BetterZR}, few-shot methods~\cite{Brown2020LanguageMA,Min2022RethinkingTR,Dong2022ASO,Ma2023FairnessguidedFP}, expert prompting~\cite{Xu2023ExpertPromptingIL}, and Chain-of-Thought (CoT)~\cite{Wei2022ChainOT, Zhang2022AutomaticCO}, with extensions like self-consistency~\cite{Wang2022SelfConsistencyIC}, Tree-of-Thought (ToT)~\cite{Yao2023TreeOT}, and Graph-of-Thought (GoT)~\cite{Besta2023GraphOT, Yao2023BeyondCE, Lei2023BoostingLR} for more complex structures.  Lately, many analogous methods have been shown to improve the performance of LMMs as well: VidIL~\cite{Wang2022LanguageMW}, DDCoT~\cite{Zheng2023DDCoTDC}, Multimodal-CoT~\cite{Zhang2023MultimodalCR, Wang2023TSciQTM}, and CCoT~\cite{MitraCCoT}.

Our work builds off of research showing that internal representations of LLMs or vision models called task vectors~\cite{Todd2023FunctionVI, Hendel2023InContextLC, Hojel2024FindingVT} (or alternatively: function vectors) can encapsulate tasks that are strictly text or strictly images given a few in-context learning (ICL) examples. This paired with recent demonstrations of multimodal ICL in LMMs both with~\cite{Doveh2024TowardsMM-ICL, Zhao2023MMICLEV} and without finetuning~\cite{Sun2023Emu2, Bai2023QwenVLAF, Laurenccon2023IDEFICS}  motivates our work which shows the existence of implicit representations called Multimodal Task Vectors ({\smodel}) that enable multimodal many-shot ICL for finetuning-free model adaptation.

\minisection{Large Multimodal Models (LMMs)} The state-of-the-art performance of LMMs~\cite{liu2023llava, liu2023llava15, Alayrac2022FlamingoAV, li2023blip2,instructblip, zhu2023minigpt4, Ye2023mPLUGOwlME, Ye2023mPLUGOwl2RM, Bai2023QwenVLAF, Gong2023MultiModalGPTAV, Driess2023PaLMEAE} on a wide variety of multimodal tasks stems largely from their combination of LLMs' powerful reasoning capabilities ~\cite{Raffel2019ExploringTL, Chowdhery2022PaLMSL,Tay2022UL2UL} with existing VL models. While these previous contrastive VL methods~\cite{radford2021clip,blip,li2023blip2} were significant in connecting vision and language, LMMs' generative reasoning over both vision and language makes them applicable to more general downstream multimodal tasks such as visual question-answering \cite{antol2015vqa, Hudson2019GQAAN, Saikh2022ScienceQAAN, Marino2019OKVQAAV, Jia2021ScalingUV, He2019MomentumCF, Gurari2018VizWizGC} and object identification and localization~\cite{Flowers, Birds, Lin2014MSCOCO, krishna2017visual}. Similar to LMMs, \textit{Visual Programmatic Models (VPMs)} are another class of multimodal methods that makes use of code generation as a proxy for visual reasoning. These include methods like ViperGPT \cite{Suris2023ViperGPTVI}, VisProg~\cite{Gupta2022VisualPC}, and CodeVQA~\cite{Subramanian2023ModularVQ}), among many others~\cite{Schick2023ToolformerLM, Lu2023ChameleonPC, Shen2023HuggingGPTSA, Qin2023ToolLLMFL, Wu2023VisualCT}. However, VPMs largely fall behind LMMs because they do not directly reason over both images and text and are limited by the APIs and models they are given access to in their limited context lengths. 

Indeed context length represents one limitation on LMMs for effectively using few-shot prompting methods such as in-context learning~\cite{Brown2020OGICL}. Another key challenge is that most LMMs are pre-trained on single text-image pair data. Recently, there has been increased interest in LMM base models that pretrain on interleaved text-image data~\cite{Bai2023QwenVLAF, Sun2023Emu2, Alayrac2022FlamingoAV, Laurenccon2024Idefics2, Jiang2024MANTISIM}, making effective in-context learning without finetuning a possibility. Our work thus looks to answer the question of whether implicit representations of ICL tasks exist in the attention heads of LMMs and whether these representations can enhance LMMs' zero-shot and few-shot capabilities.





==> archive/3_methods.tex <==
\section{{\model} ({\smodel})}

To address the challenge of performing multimodal, many-shot in-context learning, we demonstrate the existence of task vectors in LMMs and then leverage them for multimodal many-shot ICL. We begin by describing the standard multimodal few-shot ICL setting (\Secref{sec:MTV:preliminaries}). We then introduce our two-step approach: first is to extract the set of LMM attention heads that best encode the many-shot ICL task (\Secref{sec:MTV:mtvextract}), and second is patching the mean activations from doing many-shot ICL into these heads for downstream inference (\Secref{sec:MTV:mtvapp}). The method is illustrated~\figgref{fig:overview}.

\subsection{Preliminaries}
\label{sec:MTV:preliminaries}


In this work, we use a multimodal ICL setting, a version that is similar to the text-only ICL framework, except it can be applied to LMMs as they can reason over both images and text. Particularly, a few-shot multimodal ICL input $I_\mathrm{few}$ consists of multimodal in-context examples $E$--- in the form of randomly-selected query-response pairs $(q_i: r_i)$, and $Q$---the query to be answered by the LMM. Similar to the standard text-only ICL, the purpose of multimodal ICL is to learn the relationships between the in-context examples to generate a response $R$ to the input query. A few-shot multimodal ICL input is given as:
\nolinebreak
\begin{align}
   I_\mathrm{few} &= \text{``[$E$] [$Q$]''} \\
                  &= \text{``[$(q_1: r_1), (q_2: r_2), \ldots, (q_n: r_n)$] [$Q$]''}
\end{align}

We note how the in-context examples are passed sequentially to the LMM. This necessarily restricts multimodal ICL to being few-shot due to the limitation of context length (i.e., $n$ is a small number). And since images require longer embeddings, it becomes clear that some additional method is required to surpass few-shot ICL and enable \textit{many-shot} ICL in LMMs.

%Little summary paragraph before going into the details
In our work, we prove the existence of {\smodel}, which are task vectors---or specialized sets of activations extracted from an LMM's attention heads---that encode a multimodal in-context task. We then use this internal representation to encode many shots of multimodal ICL examples. Notably, our method does not require finetuning. Furthermore, because the {\smodel} is patched implicitly into the attention heads of the LMM, our method requires no input tokens and is thus not limited by the model's inherent context length. Overall, {\model} are implicit representations of LMMs using many text-image examples. These {\smodel} can then be applied to downstream inference, enabling many-shot ICL for LMMs on a variety of VL tasks, such as VQA or object identification.


\subsection{Step 1: Task Vector Extraction}
\label{sec:MTV:mtvextract}

Past work has shown the effectiveness of selecting a task vector exclusively from the last token of the model~\cite{Todd2023FunctionVI, Hendel2023InContextLC}. More recently, it has been shown that selecting a \textit{set} of task vectors to encode an ICL task is better in practice~\cite{Hojel2024FindingVT}. In our case, we look to find the optimal set of multimodal task vectors in an LMM to encode a multimodal, many-shot task.

We first introduce some notation similar to that presented in~\cite{Hojel2024FindingVT}. Given a task $j$, consider the mean activation $\mu_{i, j}$ for each activation head in the LMM. The index $i$ uniquely identifies each attention head as follows:
\nolinebreak
\begin{equation}
    i = (l,m,k)
\end{equation}

\quad Where $l$ is the layer number in the LMM, $m$ is the specific attention head with layer $l$, and $k$ is the token position within the input sequence processed by head $m$ in layer $l$. We further denote the activation of each head $i$ for task $j$ as $z_{i,j}$. The mean activation $\mu_{i, j}$ is then computed as the average of the activations outputted when the model processes examples of task $j$:
\nolinebreak
\begin{equation}
    \mu_{i, j} = \mathbb{E}[{z_{i, j}}]
\end{equation}

To find the optimal set of \roei{multimodal} task vectors to utilize for inference $z_j$, we leverage the REINFORCE~\cite{Williams2004SimpleSG} algorithm. The algorithm adjusts the probabilities of selecting specific activations for the \roei{multimoda} task vector using a policy gradient method. 

Each component $\mu_{i, j}$ is considered for inclusion in the multimodal task vector $z_j$ based on Bernoulli random variable $\alpha_{i,j}\sim \mathrm{Bernoulli}(\sigma(\theta_{i,j}))$, where $\theta_{i,j}$ is a learned parameter. Thus, the set of task vectors $z_j$ for task $j$ is given by:\roei{why zj is mentioned here...how is this different from the zi,j from above?}
\nolinebreak
\begin{equation}
    z_{j} = \{ \mu_{i, j} | \alpha_{i,j}=1\}
\end{equation}
Now, we describe the data used to learn this parameter $\theta$. We perform many-shot multimodal ICL by preparing a few-shot input $I_i$ for \textit{each iteration} $t$ of the learning process of $\theta$. Each $I_i$ is prepared like $I_\mathrm{few}$ described earlier (\Secref{sec:MTV:preliminaries}) with examples selected at random and formatted along with a query $Q_i$.
\nolinebreak
\begin{equation}
   I_i = \text{``[$(q_1: r_1), (q_2: r_2), \ldots, (q_n: r_n)$] [$Q_i$]''}
\end{equation}
Thus, for $T$ iterations of REINFORCE, we have a many-shot multimodal dataset and set of responses $R_\mathrm{many}$:
\nolinebreak
\begin{align}
   I_\mathrm{many} &= (I_1, I_2,\ldots, I_T) \\
   R_\mathrm{many} &= (R_1, R_2,\ldots, R_T)
\end{align}
% \begin{empheq}[box=\fbox]{align}
%    I_\mathrm{many} &= (I_1, I_2,\ldots, I_T) \\
%    R_\mathrm{many} &= (R_1, R_2,\ldots, R_T)
% \end{empheq}

\roei{ you defined I-many and R-many, but I don't see where you are using them below...}

For a visual depiction of this, refer to~\figgref{fig:overview}. 

The loss function $L_t(\theta)$ at iteration $t$ associated with task $j$ is defined as the expected loss over outputs produced when the model $F$ uses the task vectors $z_j$:
\begin{equation}
   L(\theta) = \mathbb{E}_{z_j \sim p_\theta} \left[ L(R_t, F(I_t | z_j)) \right] \\
\end{equation}
where $I_t = \text{``[$(q_1: r_1), (q_2: r_2), \ldots, (q_n: r_n)$] [$Q_t$]''}$ is a set of randomly-selected few-shot examples and the query $Q_t$. The algorithm then updates $\theta$ with the following estimated gradient:
\begin{equation}
   \nabla_\theta L(\theta) = \mathbb{E}_{z_j \sim p_\theta} \left[ L(R_t, F(I_t | z_j)) \nabla_\theta \log p_\theta(z_j) \right]\\
\end{equation}
It is essential to notice that across many iterations, $\theta$ and consequently the task vector $z_j$ is optimized to encode the ICL task outlined by orders of magnitude more examples than in few-shot ICL. \roei{put a conclusion paragraph. What you have now until this point, and what you still need to do. This should lead us to the next subsection.}

%This comes later



%Intuitively then, we would like to find task vectors that encode a multimodal task having seen many in-context learning examples, allowing for a better understanding of the underlying task for superior downstream performance.
%Describe how to calculate mean activations

%Describe how to find the heads via REINFORCE

\subsection{Step 2: Task Vector Application}

After finding our \roei{multimodal} task vector, we look to utilize it for downstream task inference. We patch the \roei{multimodal} task vector into the model, obviating the need for any context length to perform multimodal many-shot ICL. In particular, this means that the positions specified by the now optimized task vector $z_\mathrm{MTV}$ \roei{where is this defined above?} are directly replaced with the mean of the activations $\mu_{i,j}$ that were triggered when the model processed the many-shot examples for task $j$. This patched model can then process new inputs $Q_\mathrm{new}$, applying the learned {\smodel}'s behavior without needing to finetune the model or additional examples. 
\nolinebreak
\begin{equation}
    R_{new} = F(Q_{new}|z_\mathrm{MTV})
\end{equation}
The key insight of our method is the importance of $n$ (the number of examples) and $T$ (the number of iterations) during the optimization of the task vector $z_j$ to perform implicit multimodal, many-shot ICL. Recall that the number of examples in the few-shot setting, $I_\mathrm{few}$ is limited by the context length. {\model} enable an LMM to go beyond its context length to learn more nuanced properties of the task from seeing many examples.


%Describe the patching procedure

%At the end emphasize the importance
\label{sec:MTV:mtvapp}
%1. Extracting Mean Activations
%2. Finding the heads
%3. Patching

==> archive/3_methods_v2.tex <==
\section{{\model} ({\smodel})}

To address the challenge of performing many-shot multimodal in-context learning, we demonstrate the existence of multimodal task vectors in LMMs and then leverage them for many-shot multimodal ICL. We begin by describing the standard multimodal few-shot ICL setting (\Secref{sec:MTV:preliminaries}). We then introduce our two-step approach: first is to extract the set of LMM attention heads that best encode the many-shot multimodal ICL task (\Secref{sec:MTV:mtvextract}), and second is patching the mean activations from doing many-shot ICL into these heads for downstream inference (\Secref{sec:MTV:mtvapp}). The method is illustrated~\figgref{fig: overview}.

\subsection{Preliminaries}
\label{sec:MTV:preliminaries}

%In this work, we use a multimodal ICL setting, which is similar to the text-only ICL framework, except it can be applied to LMMs as they can reason over both images and text. 
In the multimodal in-context learning setting, an LMM learns a new task outlined by a set of multimodal inputs and text outputs.
We note that in-context examples are commonly passed sequentially to the LMM, necessarily restricting multimodal ICL to being few-shot due to limited context length. Furthermore, the images require longer embeddings, which means enabling many-shot ICL is even more challenging in the multimodal domain. To solve this, we utilize our method Multimodal Task Vectors---which are specialized sets of activations extracted from a model's attention heads that encode a task described by many-shot multimodal in-context learning examples.

%Particularly, a few-shot multimodal ICL input $I_\mathrm{few}$ consists of multimodal in-context examples $E$--- in the form of randomly-selected input-output pairs $(x_i: y_i)$, and $Q$---the query to be answered by the LMM. Similar to the standard text-only ICL, the purpose of multimodal ICL is to learn the relationships between the in-context examples to generate a response $R$ to the input query. A few-shot multimodal ICL input is given as:
% \nolinebreak
% \begin{align}
%    I_\mathrm{few} &= [E, Q]\\
%                   &= [(x_1: y_1), (x_2: y_2), \ldots, (x_n: y_n), Q]
% \end{align}

Recent work in the text domain has shown the effectiveness of selecting a task vector exclusively from the last token of the model~\cite{Hendel2023InContextLC,Todd2023FunctionVI}. More recently, in the image domain, it has been shown~\cite{Hojel2024FindingVT} that considering all tokens for task vector extraction using only a single-shot ICL example can enable visual prompting. In contrast, in this work we demonstrate the existence of an optimal task vector $z^\mathrm{MTV}_j$ in an LMM which can encode \textit{many-shot multimodal} ICL examples, leading to enhanced performance on vision-and-language downstream tasks. Our method makes use of the REINFORCE algorithm~\cite{Williams2004SimpleSG}, a policy optimization method that can be used to find task vectors without finetuning. We start by providing background details on how REINFORCE can be used to find task vectors and then compare it to our methodology for finding multimodal task vectors in the following sections.

%In our case, we first show the existence of an optimal set of multimodal task vectors $z_j$ in an LMM (where $j$ denotes the task) by leveraging the REINFORCE~\cite{Williams2004SimpleSG} algorithm. More importantly, we leverage {\smodel}s to enable multimodal, many-shot ICL in LMMs. 

% We first describe how REINFORCE is utilized in an image-only case as in~\cite{Hojel2024FindingVT} and then compare it to our methodology for finding multimodal task vectors. 

Prompted with an example input-output pair $(x_e, y_e)$ and a new query input $Q$ of some task $j$, a model $F$ can infer the underlying task based on the example and apply it to the query:
\nolinebreak
\begin{equation}
    R = F(x_e, y_e, Q)
\end{equation}
By doing in-context learning, the model can output response $R$ to the query $Q$ given the query's task specified by the example. Given a model, example-query prompts, and corresponding expected responses, REINFORCE returns a task vector $z_j$ that encode the underlying task $j$.
\nolinebreak
\begin{equation}
    z_j = \mathrm{REINFORCE}(F, [(x_1: y_1, Q_1), (x_2: y_2, Q_2), \ldots, (x_T: y_T, Q_T)], [R_1, R_2, \ldots, R_T]) 
\end{equation}

\quad where $T$ is the fixed number of iterations REINFORCE is run using only 1-shot per iteration. The algorithm finds task vectors by iteratively optimizing a Bernoulli distribution over the attention heads of the model as a way of selecting the set of heads that best encode the task. We describe further the underlying details of REINFORCE in~\Secref{sup:REINFORCE} in the Supplementary.

%Little summary paragraph before going into the details
In our work, we first prove the existence of {\model} ({\smodel}) in LMMs that can encode a multimodal in-context task via many in-context examples across iterations of REINFORCE. Thus, {\smodel} are a new type of task vector that views a task in-context of \textit{many other multimodal examples}, demonstrating how task vectors can be used in complex multimodal tasks without finetuning. Furthermore, because the {\smodel} is patched implicitly into the attention heads of the LMM, our method requires no input tokens and is thus not limited by the model's inherent context length. Overall, {\model} are compact, implicit representations of LMMs that can enable many-shot ICL for LMMs on a variety of VL tasks, such as VQA or object identification. Next, we demonstrate how to extract the {\smodel}.


\subsection{Step 1: Multimodal Task Vector Extraction}
\label{sec:MTV:mtvextract}

We notice that a key limitation of the standard REINFORCE formulation is the usage of only $n=1$ examples for a fixed set of $T$ iterations. This constitutes simply a few-shot ICL, one-shot at a time. However, here we show that better multimodal task vectors can be extracted by increasing the number of shots per iteration $n$, and the number of iterations used $T$. This enables a many-shot ICL paradigm that was previously limited by the context length of the LMM. 


The importance of our method is that the extracted multimodal task vector enables an LMM to use multiple multimodal ICL examples over many iterations, leading to superior performance on complex multimodal tasks. We describe the particulars of our method as follows.

We perform many-shot multimodal ICL by preparing a multiple-shot input $I_t$ for \textit{each iteration} $t$ of the REINFORCE learning process. Each $I_t$ consists of $n$ shots (where $n > 1$) of multimodal in-context examples---in the form of randomly-selected input-output response pairs $(x_i: y_i)$, and $Q_i$---the query to be answered by the LMM in that iteration.
\nolinebreak
\begin{equation}
   I_t = [(x_1: y_1), (x_2: y_2), \ldots, (x_n: y_n), Q_i]
\end{equation}
Thus, for $T$ iterations of REINFORCE, we have a many-shot multimodal dataset and set of responses $R_\mathrm{many}$ corresponding to the set of queries:
\nolinebreak
\begin{align}
   I_\mathrm{many} &= [I_1, I_2,\ldots, I_T] \\
   R_\mathrm{many} &= [R_1, R_2,\ldots, R_T]
\end{align}

Thus, our extraction of the multimodal task vector $z^\mathrm{MTV}_j$ is given as follows:
\nolinebreak
\begin{align}
    z^\mathrm{MTV}_j &= \mathrm{REINFORCE}(F, I_\mathrm{many}, R_\mathrm{many}) \\
    &= \mathrm{REINFORCE}(F, [I_1, I_2 \ldots, I_T], [R_1, R_2, \ldots, R_T]) 
\end{align}

During the extraction process, we also keep track of the mean activations $\mu_{i, j}$, which are just computed as the average of the activations for each attention head $i$ outputted when the model processes examples of task $j$:
\nolinebreak
\begin{equation}
    \forall i: \quad \mu_{i, j} = \mathbb{E}[{z_{i, j}}]
\end{equation}
Then, for conciseness, just let $\mu_j$ represent the vector of mean activations for all $i$. These will be utilized in the second step of task vector patching. For more details, see~\Secref{sup:REINFORCE} in Supplementary.

It is essential to notice that across many iterations, $z^\mathrm{MTV}_j$ and $\mu_j$ are optimized to encode the ICL task outlined by orders of magnitude more examples than in few-shot ICL. Now that we have extracted both $z^\mathrm{MTV}_j$ and $\mu_j$, we describe the patching process for downstream inference in the next section. 

% Thus far, we have shown the existence of {\model} ({\smodel}) in LMMs that encode a multimodal in-context task. The next step would be to encode many examples of multimodal ICL using this internal representation.

%The algorithm adjusts the probabilities of selecting specific activations for the multimodal task vector using a policy gradient method. 

\subsection{Step 2: Task Vector Application}
\label{sec:MTV:mtvapp}

After finding our multimodal task vector, we look to utilize it for downstream task inference. In simple terms, $\mu_j$ contains the averaged activation values learned from many-shot ICL, and $z^\mathrm{MTV}_j$ describes the optimal locations (or indices of the attention heads) in the LMM to patch those values into for a task $j$. More specifically, ``patching" the multimodal task vector involves \textit{directly replacing} each attention head $i$ in $z^\mathrm{MTV}_j$ with the mean activation accumulated during multimodal, many-shot ICL $\mu_{i,j}$. This patched model can then process new inputs $Q_\mathrm{new}$. 
\nolinebreak
\begin{equation}
    R_{new} = F(Q_{new}|z^\mathrm{MTV}_j, \mu_{j})
\end{equation}
The key insight of our method is the importance of multiple $n$ (the number of examples) and many $T$ (the number of iterations) during the optimization of the task vector $z_j$ to perform implicit multimodal, many-shot ICL without any finetuning. Recall that the context length limits the number of examples in the few-shot setting. {\model} enables an LMM to go beyond its context length to learn more nuanced properties of the task from seeing many examples. Patching the multimodal task vector into the model also obviates the need for any context length during downstream inference, actually \textit{freeing} additional context for other use (e.g. an additional prompt, more ICL examples, etc.).


==> archive/3_methods_v3.tex <==
\section{{\model} ({\smodel})}

To address the challenge of performing many-shot multimodal in-context learning, we demonstrate the existence of multimodal task vectors in LMMs and then leverage them for many-shot multimodal ICL. We begin by describing some background on multimodal ICL and task vectors (\Secref{sec:MTV:preliminaries}). We then introduce our three-step approach: first is to calculate the mean activations of the attention heads from doing many-shot ICL (\Secref{sec:MTV:mu}); second, is to extract the set of LMM attention heads locations that encode the many-shot multimodal ICL task using an adapted version of the REINFORCE~\cite{Williams2004SimpleSG}(\Secref{sec:MTV:mtvextract}); and third is to directly replace the calculated mean activation values into the LMM for a downstream task (\Secref{sec:MTV:mtvapp}). The method overview is also illustrated~\figgref{fig:overview}.

\subsection{Preliminaries}
\label{sec:MTV:preliminaries}
In the multimodal in-context learning setting, an LMM learns a new task outlined by a set of multimodal examples. The input to the LMM would be outlined as follows:
\nolinebreak
\begin{equation}
    I_\mathrm{few} = [(x_1: y_1), (x_2: y_2), \ldots, (x_n: y_n), Q]
\end{equation}
\quad where the model is prompted to answer a query $Q$ given a set of input-output examples (each $x_i$ being a multimodal input and each $y_i$ a text output).


We note that in-context examples are commonly passed sequentially to the LMM, necessarily restricting multimodal ICL to being small numbers of shots due to limited context length. Furthermore, the images require longer-token embeddings, which means enabling many-shot ICL is even more challenging in the multimodal domain. To solve this, we utilize our method Multimodal Task Vectors---which are implicit representations in the model's attention heads that encode a many-shot multimodal ICL task.


We give some background on task vectors. Given task $j$, a task vector has two parts: (1) the task vector \textbf{locations} $z_j$, which denotes a subset of the attention heads, and (2) the task vector \textbf{values} $\mu_j$, which are mean activations triggered from examples of a task. For inference, $\mu_j$ replaces the activation values of the heads in $z_j$, giving us an implicit representation of task $j$. 

In prior work~\cite{Hendel2023InContextLC,Hojel2024FindingVT,Todd2023FunctionVI}, the calculation of the mean activations $\mu_j$ and the extraction of the attention-head locations $z_j$ are used only to extract the task vector. However, we find that these two steps should be decoupled in order to better align with the downstream task. In our work, we calculate the mean activations $\mu_j$ specifically to encode a dataset of many-shot multimodal ICL examples by averaging them across multiple inference calls. Then, during the extraction of the attention-head locations $z_j$, we use a separate set of examples that are of the exact format of the downstream task for better alignment of the selected attention heads. The distinct allocation of responsibilities, wherein $\mu_j$ captures the essential information from the many-shot examples and $z_j$ identifies the specific attention head locations for the downstream task, optimizes the utilization of the encoded information at relevant locations within the model. 


These factors encapsulate the unique features of {\model} ({\smodel}) $(z^\mathrm{MTV}_j, \mu^\mathrm{MTV}_j)$. Our approach allows LMMs to actually leverage many-shot multimodal ICL examples for downstream tasks complex vision-language tasks without being limited by context length. We proceed by first demonstrating how to calculate the mean activations.

% This distribution of ``work" such that $\mu_j$ encodes the actual stored information from the examples and $z_j$ represents the attention head locations that are specific to a downstream task leads to the best usage of the information in $\mu_j$ at the right locations $z_j$.
% Building on this foundation, we advance our methodology by introducing the {\model} ({\smodel}) $(z^\mathrm{MTV}_j, \mu^\mathrm{MTV}_j)$. This approach aggregates insights from multiple inference calls, averaging over many multimodal examples 


% In our work, we calculate the {\model} ({\smodel}) $(z^\mathrm{MTV}_j, \mu^\mathrm{MTV}_j)$ by averaging \textit{many shots} of multimodal examples across multiple inference calls. This enables an LMM to utilize more examples for complex vision-language tasks without being limited by context length. First, we start by demonstrating how to extract the {\smodel}.

\subsection{Step 1: Calculate {\smodel} Mean Activations}
\label{sec:MTV:mu}

% The first step of {\smodel} is to calculate the mean activations of the LMM given a set of many-shot multimodal ICL examples for a task $j$. 
The ultimate objective of many-shot multimodal ICL is to use a large number of input-output examples when solving a task $j$. However, it is not trivial to get the LMM to see more examples during inference time than its context length allows.

To address this issue, we pass a few-shot input $I_t$ for each inference call $t$ for a total of $T > 1$ inference calls. Each $I_t$ consists of $N$ shots (where $N > 1$) of multimodal in-context examples in the form of randomly-selected input-output response pairs $(x_t: y_t)$, and $Q_t$, which is the query to be answered by the LMM in that iteration.
\nolinebreak
\begin{equation}
   I_t = [(x_1: y_1), (x_2: y_2), \ldots, (x_N: y_N), Q_t]
\end{equation}
Thus, over $T$ LMM inference calls, we have a many-shot multimodal dataset (of $nT$ examples) and a set of responses $R_\mathrm{many}$ corresponding to the set of queries:
\nolinebreak
\begin{align}
   I_\mathrm{many} &= [I_1, I_2,\ldots, I_T] \\
   R_\mathrm{many} &= [R_1, R_2,\ldots, R_T]
\end{align}

However, this dataset is still just a disconnected set of few-shot examples. Next, we would like to connect the separate examples into one unified many-shot multimodal ICL representation.

% \textit{How then, do we connect the separate examples into one unified many-shot multimodal ICL representation?}

We do this by averaging---across all $T$ inference calls and all $n$ examples per call---the activations for each attention head $i$, yielding:
% \nolinebreak
% \begin{equation}
%     \forall i: \quad \mu_{i, j} = \frac{1}{T} \sum_{t=1}^T \frac{1}{n} \sum_{n=1}^N z_{i,j,n,t}
% \end{equation}
\nolinebreak
\begin{equation}
    \forall i: \quad \mu_{i, j} = \frac{1}{T} \sum_{t=1}^T \mathbb{E}[z_{i,j} \mid I_t] = \frac{1}{T} \sum_{t=1}^T \mathbb{E}\left[z_{i,j} \mid [(x_1: y_1), (x_2: y_2), \ldots, (x_N: y_N), Q_t]\right]
\end{equation}
\quad where $z_{i,j}$ are the activations of the attention heads. 

Crucially, in this step, we have found the mean activations $\mu_{i,j}$, which encode an internal LMM representation of many shots of multimodal ICL examples. In the next subsection, we describe our methodology for selecting the set of attention heads where these mean activations will be used.

\subsection{Step 2: Extract {\smodel} Attention Head Locations}
\label{sec:MTV:mtvextract}


After Step 1, we now have mean activations for all attention heads of the LMM for a given many-shot multimodal task. Yet, we still need to find which set of attention heads $z^\mathrm{MTV}_j$ should be chosen to encode our task.


To choose the set of attention heads, we first prepare a separate set of $S$ examples specifically aligned to the format of the downstream task. For instance, if the downstream setting is a 2-way, one-shot classification task, then the $S$ examples should conform to this paradigm. For our explanation, let's consider a downstream task that is zero-shot such that there is a single query $Q_s$ and corresponding response $R_s$ for all $s \in [1, 2, \ldots, S]$. From these examples, we utilize an adapted version of the REINFORCE~\cite{Williams2004SimpleSG} algorithm---an iterative policy optimization method that can be used to find task vector locations. Given an LMM $F$, we first sample a  Bernoulli distribution over the set of attention heads. Next, we directly replace the values of the selected attention heads with the corresponding mean activations $\mu_{i,j}$. Then, after prompting the model with the query $Q_s$, we use the cross-entropy loss between the LMM's output logits and the logits of the ground-truth response $R_s$ to optimize the Bernoulli distribution. By optimizing the Bernoulli distribution across $S$ iterations, we are finding the best attention head locations $z^\mathrm{MTV}_j$ for patching in our mean activations. Finally, we can extract $z^\mathrm{MTV}_j$, the optimized set of attention heads, by sampling our optimized Bernoulli distribution.
\nolinebreak
\begin{equation}
    z^\mathrm{MTV}_j = \mathrm{MTV\_EXTRACT}(F, [Q_1, Q_2, \ldots, Q_S)], [R_1, R_2, \ldots, R_S])
\end{equation}

% Given an LMM $F$, a query $Q_s$, the corresponding response $R_s$, and the mean activations $\mu_{i,j}$, we sample a Bernoulli distribution over the set of attention heads.
% We directly replace their values with $\mu_{i,j}$, the corresponding mean activation for each $i$ in the sampled set of attention heads.
% After prompting the model with $Q_s$, we use the cross-entropy loss between the LMM's output logits and the ground truth logits $R_s$ to optimize the Bernoulli distribution. By optimizing the Bernoulli distribution, we are finding the best attention head locations $z^\mathrm{MTV}_j$ for patching in our mean activations. 
% After $S$ iterations, we can then get $z^\mathrm{MTV}_j$ by sampling our optimized Bernoulli distribution.

We describe further the underlying details of our adapted MTV\_EXTRACT algorithm in~\Secref{sup:REINFORCE} of the Supplementary. Having found $z^\mathrm{MTV}_j$ and $\mu_{i,j}$, we describe in what follows, the final procedure to use {\smodel} for inference.

\subsection{Step 3: Multimodal Task Vector Application}
\label{sec:MTV:mtvapp}
After we have identified a set of attention heads $z^\mathrm{MTV}_j$, it is straightforward to apply {\smodel} for inference. We denote the set of mean activations $z^\mathrm{MTV}_j$ as follows $\mu^\mathrm{MTV}_j = \{\mu_{i,j} | \forall i \in z^\mathrm{MTV}_j\}$.

To run downstream inference on a new query $Q_\mathrm{new}$ with our model $F$, we directly replace the values of attention heads $z^\mathrm{MTV}_j$ with $\mu^\mathrm{MTV}_j$ and produce the following response $R_\mathrm{new}$:
\nolinebreak
\begin{equation}
    R_\mathrm{new} = F(Q_{new}|z^\mathrm{MTV}_j, \mu^\mathrm{MTV}_j)
\end{equation}
$R_\mathrm{new}$ is thus a response generated using many shots of multimodal examples as implicit context via {\smodel}. The key insight of our method is the importance of $N$ (the number of multimodal examples) and many $T$ (the number of iterations) during the calculation of {\smodel}. Recall that the context length usually limits the number of examples in the few-shot setting. {\model} enables an LMM to go beyond its context length to learn more nuanced properties of the task from seeing many examples. Insertion of {\smodel} directly into the LMM also obviates the need for any context length during downstream inference, actually \textit{freeing} additional context for other use (e.g. an additional prompt, more ICL examples, etc.).

% \subsection{Step 2: Task Vector Application}
% \label{sec:MTV:mtvapp}

% After finding our multimodal task vector, we look to utilize it for downstream task inference. In simple terms, $\mu_j$ contains the averaged activation values learned from many-shot ICL, and $z^\mathrm{MTV}_j$ describes the optimal locations (or indices of the attention heads) in the LMM to patch those values into for a task $j$. More specifically, ``patching" the multimodal task vector involves \textit{directly replacing} each attention head $i$ in $z^\mathrm{MTV}_j$ with the mean activation accumulated during multimodal, many-shot ICL $\mu_{i,j}$. This patched model can then process new inputs $Q_\mathrm{new}$. 
% \nolinebreak
% \begin{equation}
%     R_{new} = F(Q_{new}|z^\mathrm{MTV}_j, \mu_{j})
% \end{equation}
% The key insight of our method is the importance of multiple $n$ (the number of examples) and many $T$ (the number of iterations) during the optimization of the task vector $z_j$ to perform implicit multimodal, many-shot ICL without any finetuning. Recall that the context length limits the number of examples in the few-shot setting. {\model} enables an LMM to go beyond its context length to learn more nuanced properties of the task from seeing many examples. Patching the multimodal task vector into the model also obviates the need for any context length during downstream inference, actually \textit{freeing} additional context for other use (e.g. an additional prompt, more ICL examples, etc.).


==> figs/fig3_efficiency.tex <==
% \begin{figure}[t]
%     \centering
%     \includegraphics[width=0.80\linewidth]{figs/plot3.png}
%     \caption{
%     \textbf{Efficiency:} We show that even though {\smodel} is encoding 400 multimodal ICL examples, it still is less runtime and compute intensive than 8-shot and 16-shot multimodal ICL.
%     }
%     \label{fig:efficiency}
%     \vspace{-0.4cm}
% \end{figure}


==> sec/6_additional_sections.tex <==
\section{Limitations}
\textbf{CCoT Template - To Be Edited}
In this work, we present a zero-shot Chain-of-Thought prompting method that utilizes scene-graph representations for multimodal and compositional visual reasoning tasks. We demonstrate improved performance on several different models and benchmarks. Nevertheless, our work has a central limitation. While extending context length is an active field of research, our method is limited by the current context lengths of the LLMs being used by the LMMs. Additionally, scene graphs are not particularly useful representations when performing multimodal tasks that emphasize language over visual reasoning, such as document understanding. Finally, we do not anticipate negative impacts of this work, but, as with any machine learning method, we recommend exercising caution.


